R-CHECK: A Model Checker for Verifying Reconfigurable MAS

Reconfigurable multi-agent systems consist of a set of autonomous agents, with integrated interaction capabilities that feature opportunistic interaction. Agents seemingly reconfigure their interactions interfaces by forming collectives, and interact based on mutual interests. Finding ways to design and analyse the behaviour of these systems is a vigorously pursued research goal. We propose a model checker, named R-CHECK, to allow reasoning about these systems both from an individual- and a system- level. R-CHECK also permits reasoning about interaction protocols and joint missions. R-CHECK supports a high-level input language with symbolic semantics, and provides a modelling convenience for interaction features such as reconfiguration, coalition formation, self-organisation, etc.

==> tex/background.tex <==
%% !TEX root = ../main.tex
\section{Transition systems}\label{sec:bck}

%We unify notations and give the necessary background. 

%\subsection{Doubly-Labeled Transition Systems and Discrete Systems}

A \emph{Doubly-Labeled Transition System} (DLTS) is
$\mathcal{T}=\langle \Sigma,\Upsilon,S, \allowbreak S_0,R,L\rangle$,
where $\Sigma$ is a \emph{state alphabet}, $\Upsilon$ is a
\emph{transition alphabet}, $S$ is a set of states, $S_0\subseteq S$
is a set of initial states, $R\subseteq S\times \Upsilon \times S$ is
a transition relation, and $L:S\rightarrow \Sigma$ is a labelling
function.

A \emph{path} of a transition system $\mathcal{T}$ is a maximal sequence of states and transition labels $\sigma=s_0,a_0,s_1,a_1,\ldots$ such that $s_0\in S_0$ and 
for every $i\geq 0$ we have $(s_i,a_i,s_{i+1})\in R$. 
We assume that for every state $s\in S$ there are $a\in \Upsilon$ and
$s'\in S$ such that $(s,a,s')\in R$. 
Thus, a sequence $\sigma$ is maximal if it is infinite.
If $|\Upsilon|=1$ then $\mathcal{T}$ is a \emph{state-labeled system} and if $|\Sigma|=1$ then $\mathcal{T}$ is a \emph{transition-labeled system}. 

We introduce \emph{Discrete Systems} (DS) that represent state-labeled systems symbolically.
A DS is $\mathcal{D} = \langle \mathcal{V}, \theta, \rho \rangle$, where the components of
$\mathcal{D}$ are as follows:
\begin{itemize}[label={$\bullet$}, topsep=0pt, itemsep=0pt, leftmargin=10pt]
\item
  $\mathcal{V} = \set{v_1,...,v_n}$: A finite set of typed variables.  
  Variables range over discrete domains, e.g., Boolean or Integer.
A \emph{state} $s$ is an interpretation of  $\mathcal{V}$,
  i.e., if $D_v$ is the domain of $v$, then $s$ is in
  $\prod_{v_i\in \mathcal{V}} D_{v_i}$.

%  We assume some underlying first-order language over $\mathcal{V}$ that
%  includes (i) \emph{expressions} constructed from the variables in
%  $\mathcal{V}$, (ii) \emph{atomic formulas} that are either Boolean variables
%  or the application of different predicates to expressions, and
%  (iii) \emph{assertions} that are first-order formulas constructed from
%  atomic formulas using Boolean connectives or quantification of
%  variables. 
%  Assertions, also sometimes called \emph{state formulas}, characterize
%  states through restriction of possible variable values in them.
\item
  $\theta$ : This is an
  assertion over $\mathcal{V}$ characterising all the initial states of the
  DS.  
  A state is called \emph{initial} if it satisfies $\theta$.
\item
  $\rho$ : A \emph{transition relation}. 
  This is an assertion $\rho(\mathcal{V}\cup\mathcal{V}')$, where $\mathcal{V}'$ is a primed
  copy of variables in $\mathcal{V}$. The transition relation $\rho$
  relates a state $s\in\Sigma$ to its \emph{$\mathcal{D}$-successors}
  $s'\in\Sigma$, i.e., 
  $(s,s')\models \rho$, where $s$ is an interpretation to
  variables in $\mathcal{V}$ and $s'$ is for variables in $\mathcal{V}'$.
\end{itemize}

The DS ${\mathcal{D}}$ gives rise to a state-labeled transition system $\mathcal{T}_{\mathcal{D}}=\langle\Sigma,\{1\},T,T_0,R\rangle$, where $\Sigma$ and $T$ are the
set of states of $\mathcal{T}_\mathcal{D}$, $T_0$ is the set of
initial states, and $R$ is the set of triplets $(s,1,s')$ such that
$(s,s')\models \rho$. Clearly, the paths of ${\mathcal{T}}_\mathcal{D}$ are exactly the
 paths of $\mathcal{D}$, but the size of $\mathcal{T}_\mathcal{D}$ is 
exponentially larger than the description of $\mathcal{D}$.

A common way to translate a DLTS into a DS, which we adapt
and extend below, would be to include 
additional variables that encode the transition alphabet.
Given such a set of variables $\mathcal{V}_\Upsilon$, an assertion
$\rho(\mathcal{V} \cup \mathcal{V}_\Upsilon \cup \mathcal{V}')$ characterises
the triplets $(s,\upsilon,s')$ such that $(s,\upsilon,s') \models
\rho$, where $s$ supplies the interpretation to $\mathcal{V}$, $\upsilon$
to $\mathcal{V}_\Upsilon$ and $s'$ to $\mathcal{V}'$.


==> tex/informal.tex <==
%% !TEX root = ../main.tex
\section{An informal overview}\label{sec:overview}%\marginpar{Y: still didn't inject the example}
We use a collaborative-robot scenario to informally illustrate the
 distinctive features of our formalism and we later formalise it in Section~\ref{sec:exp}.
The scenario is based on Reconfigurable Manufacturing Systems (RMS)~\cite{rms1,rms2},
where assembly product lines coordinate autonomously with different
types of robots to produce products. 


In our formalism, each agent has a local state
consisting of a set of variables whose values may change due to
either contextual conditions or side-effects of
interaction. The external behaviour of an agent is only represented by the messages it
exposes to other agents while the local one is represented by changes to its
state variables. These variables are initialised by initial conditions
and updated by send- and receive- transition relations.
In our example, a product-line agent initiates different production
procedures based on the assignment to its product variable $\qt{\msf{prd}}$,
which is set by the operator, while it controls the progress of its status variable
$\qt{\msf{st}}$ based on interactions with other robots.
Furthermore, a product-line agent is characterised:
(1) externally only by the recruitment and assembly messages it  
sends to other robots and
(2) internally by a sequence of assignments to its local variables.

Before we explain the send- and receive- transition relations and show
the dynamic reconfiguration of communication interfaces we need to
introduce a few additional features. 
We assume that there is an agreed set of \emph{channels/links} $\schan$ that includes a unique
broadcast channel $\star$.
Broadcasts have non-blocking send and blocking receive while
multicasts have blocking send and receive.
In a broadcast, receivers (if exist) may anonymously receive a
message when they are interested in its values and when they satisfy
the send guard.
Otherwise, the agent does not participate in the interaction either
because they cannot (do not satisfy the guard) or because they are not
interested (make an idle transition).
In multicast, all agents connected to the multicast channel must
participate to enable the interaction.
%Broadcast is used when agents are unaware of each other and possibly sharing some resources
%while multicast is used to capture a more structured interaction where
%agents have dedicated links to interact.
For instance, recruitment messages are broadcast because a line agent
assumes that there exist enough robots to join the team while assembly messages
are multicast because they require that the whole connected team is ready to
assemble the product.

Agents dynamically decide (based on local state) whether they can
use/connect-to multicast channels while the broadcast channel is always available. 
Thus,
initially, agents may not be connected to any channel, except for the
broadcast one $\msf{\star}$.
These channels may be learned using broadcast messages
and thus a structured communication interface can be built at run-time, starting
from a (possibly) flat one. 

Agents use messages to send selected data and specify
how and to whom.
Namely, the values in a message specify what is exposed to the others;
the channel specifies how to coordinate with others; and a send
guard specifies the target.
Accordingly, each message carries an assignment to a set of agreed
\emph{data variables} $\sdat$, i.e., the exposed data;  a
channel $\msf{\chan}$; and a send guard $\pfunc{g}{s}{}$.
In order to write meaningful send guards, we assume a set of
\emph{common variables} $\scv$ that each agent stores locally and
assigns its own information (e.g., the type of agent, its location,
its readiness, etc.). Send guards are expressed in terms of conditions
on these variables and are evaluated per agent based on their assigned
local values. 
Send guards are parametric to the local state of the sender
and specify what assignments to common variables a potential receiver
must have.
For example, an agent may send a dedicated link name to a selected set
of agents by assigning a data variable in the communicated message and
this way a coalition can be built incrementally at run-time.
In our RMS, the send guard of the recruitment message specifies
the types of the targeted robots while the data values expose the
number of required robots per type and a dedicated multicast link to
be used to coordinate the production. 

Targeted agents may use incoming messages to update their
states, reconfigure their interfaces, and/or adapt their behaviour.
In order to do so, however, agents are equipped with receive guards $\pfunc{g}{r}{}$; 
that might be parametrised to local variables and channels, and thus
dynamically determine if an agent is connected to a given channel. 
The interaction among different agents is then derived based on send- and receive-
transition relations.
These relations are used to decide when to send/receive a message and what are the
side-effects of interaction. 
Technically, every agent has a send and a receive transition relation.
%, each defined as a disjunction of guarded commands.
Both relations are parameterised by the state variables of the agent,
the data variables transmitted on the message, and by the channel name.
A sent message is interpreted as a joint transition between the send
transition relation of the sender and the receive transition relations of all
the receivers.
For instance, a robot's receive guard specifies that other than
the broadcast link it is also connected to a multicast link that matches the current value of
its local variable $\qt{\msf{lnk}}$. The robot then uses its receive transition relation
to react to a recruitment message, for instance, by assigning to its $\qt{\msf{lnk}}$ the
link's data value from the message.

Furthermore, in order to send a message the following has to happen.
The send transition relation of the sender must hold on: a given state of the sender,
a channel name, and an assignment to data variables.
If the message is broadcast,
all agents whose assignments to common variables satisfy the
send guard jointly receive the message, the others discard it.
If the message is multicast, all connected agents must satisfy the
send guard to enable the transmission (as otherwise they block the
message).
In both cases, 
sender and receivers execute their send- and receive-transition
relations jointly.
The local side-effect of the message takes into account the origin
local state, the channel, and the data.
In our example, a (broadcast) recruitment 
message is received by all robots that are not assigned to other teams (assigned ones  
discard it) and as a side effect they connect to a multicast
channel that is specified in the message.
A (multicast) assembly message can only be sent when the whole 
recruited team is ready to receive (otherwise the message is blocked)
and as a side effect the team proceeds to the next production stage. 

Clearly, the dynamicity of our formalism stems from the fact that we base
interactions directly over the evolving states of the different agents 
rather than over static notions of network connectivity as of existing approaches. 


==> tex/relatedwork.tex <==
% !TEX root = ../main.tex
\section{Related work}\label{sec:rel}

%\marginpar{Y: compare with respect to other models arising in verification and concurrency theory communities}
%
\paragraph*{System frameworks}
The modelling of computer systems in terms of interacting and distributed components is a well established approach in the area of formal verification that has recently been imported to multi-agent settings~\cite{Woo02,WGHMPT16,GHW17,KL17a,KL17b}.
One of the most successful formalisms in this area is the one of Reactive Modules~\cite{AH99b}, a high-level language for the specification of components capabilities in terms of guarded commands: variable assignment rules that activate/deactivate according to a guarded predicate evaluated on the current state of the system.

Antithetical to the traditional communication framework, the interaction among components is based exclusively on shared variables, whereas the message-exchange is assumed both implicit and instantaneous.
More recently, an extension to \emph{Dynamic Reactive Modules}~\cite{FHNPSV11} accounts for communication reconfigurability, where processes can evolve their set of guarded commands, as well as being created or terminated.
Other extensions of reactive modules account for scenarios in which variables are not visible to all the components~\cite{GPW18}, or such visibility is dynamically disclosed or concealed by the controller itself~\cite{BBDM19}, again allowing the communication mechanism to reconfigure.

%\marginpar{Y: compare with other existing logics and justify the need for another logic}
%
\paragraph*{Logics}
In reactive modules verification, the specification language for system correctness is usually logic-based.
In particular, LTL and CTL like languages are well established formalisms for the representation of temporal properties in systems executions.
However, such languages are not suitable to specify properties for the modalities on which transitions among systems states are triggered.
Therefore, in order to predicate over the message-passing architecture, one has to consider extensions or variations that are capable to constrain the transition relation of systems.
Existing languages of this kind include \emph{Propositional Dynamic Logic}~\cite{FL79} and \emph{modal $\mu$-calculus}~\cite{Koz83}.

Unfortunately, these languages are still limited for our purpose, as they treat the transition labels as atomic objects, whereas our system models mount complex and structured observations on which designers are willing to predicate on.
In order to verify such articulated properties along them, we need a modal language whose modalities adapt over the space of possible observations.
As we show in here, such extension comes with an unavoidable price in the complexity of the model-checking problem.




==> tex/varstyles.tex <==
%% !TEX root = ../main.tex
\newcommand{\sqt}[1]{`{#1}'}
\newcommand{\keep}{\mbox{\sc keep}}
% agents
\newcommand{\agent}[1]{\rulename{\textbf{#1}}}
\newcommand{\lineagent}{\agent{Line}}
\newcommand{\taagent}{\agent{t1}}
\newcommand{\tbagent}{\agent{t2}}
\newcommand{\tcagent}{\agent{t3}}

% variable types macros
\newcommand{\varcommon}[1]{\footnotesize{\text{@}}\mathsf{#1}}
\newcommand{\vardata}[1]{\rulename{#1}} 
\newcommand{\varlocal}[1]{\mathsf{#1}}
\newcommand{\val}[1]{{\small{\texttt{#1}}}}

% common variables
\newcommand{\typecvar}{\varcommon{type}}
\newcommand{\assigncvar}{\varcommon{asgn}}
\newcommand{\readycvar}{\varcommon{rdy}}

% data variables
\newcommand{\msgdvar}{\vardata{msg}}
\newcommand{\lnkdvar}{\vardata{lnk}}
\newcommand{\nodvar}{\vardata{no}}

% line variables
\newcommand{\stlvar}{\varlocal{st}}
\newcommand{\lnklvar}{\varlocal{lnk}}
\newcommand{\prdlvar}{\varlocal{prd}}
\newcommand{\stagelvar}{\varlocal{stage}}
\newcommand{\typelvar}{\varlocal{ltype}}
\newcommand{\assignlvar}{\varlocal{lasgn}}
\newcommand{\readylvar}{\varlocal{lrdy}}

% variable values
\newcommand{\taval}{\val{t1}}
\newcommand{\tbval}{\val{t2}}
\newcommand{\tcval}{\val{t3}}
\newcommand{\teamval}{\val{team}}
\newcommand{\assembleval}{\val{asmbl}}
\newcommand{\formval}{\val{form}}
\newcommand{\pendval}{\val{pnd}}
\newcommand{\recval}{\val{rcrt}}
\newcommand{\stageoneval}{\val{stg1}}
\newcommand{\stagetwoval}{\val{stg2}}
\newcommand{\startval}{\val{strt}}
\newcommand{\recother}{\val{rec\_oth}}

==> tex/verification.tex <==
%% !TEX root = ../main.tex
%\subsection{Computational Complexity}\label{sec:upper}
%\paragraph{The Complexity of Reasoning}
%\paragraph{\bf Satisfiability}\label{sec:sat}
\begin{theorem}\label{thm:satisfiability}
The satisfiability problem of \ltal is \pspace-complete with respect to 
$\size{\phi}$, $\size{\sysvar},\ \size{\sdat},\ \log{\size{\schan}},\ 
\log{\size{K}}$ and \expspace with respect to $\size{\scv}$. 
\end{theorem}
%\begin{proof}
%By Corollary~\ref{cor:1}, given a formula $\phi$, we can construct a
%B\"uchi automaton $A_n$ of size $\size{Q_n}.\size{\delta_n}$ that
%accepts precisely the computations that satisfy $\phi$. Thus, $\phi$
%is satisfiable iff $A_n$ is nonempty. The satisfiability problem is
%reduced to the nonemptiness of $A_n$. The nonemptiness of a B\"uchi
%automaton is tested in nondeterministic logarithmic space and we get a
%polynomial space algorithm with respect to $\size{\phi}$,
%$\size{\sysvar},\ \size{\sdat},\ \log{\size{\schan}},\ \log{\size{K}}$
%and EXPSPACE with respect to $\size{\scv}$. The algorithm constructs
%$A_n$ on-the-fly. The hardness argument~\cite{sistlac85} can be proved
%by the fact that any PSPACE-hard problem can be reduced to the
%satisfiability problem.  
%\end{proof}

%\paragraph{\bf Model Checking}\label{sec:ver}
\begin{theorem}\label{thm:modcheck}
The model-checking problem of \ltal is \pspace-complete with respect to $\size{Sys}$, $\size{\phi}$, $\size{\sysvar},\ \size{\sdat},\ \log{\size{\schan}},\\ \log{\size{K}}$ and \expspace with respect to $\size{\scv}$. 
\end{theorem}
%\end{remark}
%\begin{proof}
%Given a finite state system $Sys=\conf{\sysvar\coma\rho\coma\theta}$ and a set of assertions on state variables $\sysvar$, on $\schan,\ {\sdat},\ K$, and on $cv_1,\dots cv_n$. We assume $\rho$ to be total and then we can construct an automaton 
%$A_s=\conf{S,\Sigma, M, S_0, \delta_s, S}$ such that the set of states
%$S$ is the set of possible interpretations of the variables in
%$\sysvar$. The set of initial states $S_0$ is the set of states $s$
%such that $s\models \theta$, i.e., $S_0=\set{s\models {\theta}}$,
%$\Sigma=\Exp{\sysvar}$, and  $M=\schan\times\Exp{\sdat}\times K\times
%\dexp{\scv}$. We have that $\delta_s(s,\sigma,m)=\set{s':
%  \tuple{s,\sigma,m,s'}\models \rho}$ and $\emptyset$ otherwise. The
%number of states in the transition system may be exponentially larger
%than the description of $Sys$.
%
%$Sys$ satisfies $\phi$ iff all the computations of $Sys$ satisfy
%$\phi$, thus $\lang{A_s}\subseteq \lang{A_{\phi}}$. This is equivalent
%to check $\lang{A_s}\cap\lang{A_{\neg \phi}}=\emptyset$. Since our
%formulas are in positive normal form, $\neg\phi$ can be obtained from
%$\phi$ by $\overline{\phi}$. By Corollary~\ref{cor:1}, we have that
%$A_{\neg\phi}$ has $\Exp{\bigo{\size{\phi}}}$ states and
%$\size{A_{\neg\phi}}$ is in
%$\bigo{\size{\schan}.\size{K}.\Exp{\size{\phi}+\size{\sysvar}+\size{\sdat}+\Exp{\size{\scv}}}}$. The
%model checking problem can be reduced to the nonemptiness problem of
%the intersection of $A_{s}$ and $A_{\neg\phi}$. Since all states in
%$A_{s}$ are accepting, the construction of $A_{s,\neg\phi}$ is the
%product of $A_{s}$ with $A_{\neg\phi}$. We have that $A_{s,\neg\phi}$
%has $\Exp{\bigo{\size{Sys}+\size{\phi}}}$ states. Hence, $\size{A_{s,
%    \neg\phi}}$ is in
%$\bigo{\size{\schan}.\size{K}.\Exp{\size{\phi}+\size{Sys}+\size{\sysvar}+\size{\sdat}+\Exp{\size{\scv}}}}$. We
%have that $A_{s,\neg\phi}$ can be constructed on-the-fly and a
%membership in PSPACE with respect to $\size{Sys}$, $\size{\phi}$,
%$\size{\sysvar},\ \size{\sdat},\ \log{\size{\schan}},\ \log{\size{K}}$
%and a membership in EXPSPACE with respect to $\size{\scv}$ follow from
%the membership in NLOGSPACE of the nonemptiness problem for
%NBW. Checking that $Sys\models\phi$ is in
%$\bigo{\log\size{\schan}+\log\size{K}+{\size{\phi}+\size{Sys}+\size{\sysvar}+\size{\sdat}+\Exp{\size{\scv}}}}$. The
%PSPACE hardness~\cite{sistlac85} can be proved by a generic reduction
%from polynomial-space to Turing-machines. 
%\end{proof}

\newcommand{\lowerbound}{

We now investigate the hardness of \ltal satisfiability and model-checking by showing a reduction from EXPSPACE tiling problem~\cite{Wang90,Boas97} to satisfiability and model-checking, providing EXPSPACE hardness. 

\begin{theorem}[hardness]
	\label{thm:hardness}
	The satisfiability and model-checking problems for properties in \ltal are EXPSPACE-hard.
\end{theorem}

\begin{proof}
  The proof is in Appendix~\ref{sec:appendix}.
  Let $\Exp{m}$ be the width of the required tiling.
  The crux of the proof is in checking that two tiles that are
  $\Exp{m}$ apart from each other satisfy some consistency rules.
  We use common variables that can describes tiles and a number
  counting to at most $\Exp{m}-1$.
  A predicate over the common variables has a set of possible truth
  assignments to these variables.
  Thus, we can think about the predicate as a relation between
  locations (modulo $\Exp{m}$) and tiles.
  We use the observation descriptors to force the predicates to
  specify that this relation is actually a function and so that the
  function memorizes a full row in the tiling (i.e., $\Exp{m}$ tiles).
  Then, by looking on the predicate we can compare the current tile to
  a tile that appeared $\Exp{m}$ locations ago. 
\end{proof}
}

%\lowerbound

